DexCtrl: Towards Sim-to-Real Dexterity with Adaptive Controller Learning

Dexterous manipulation has seen remarkable progress in recent years, with policies capable of executing many complex and contact-rich tasks in simulation. However, transferring these policies from simulation to real world remains a significant challenge. One important issue is the mismatch in low-level controller dynamics, where identical trajectories can lead to vastly different contact forces and behaviors when control parameters vary. Existing approaches often rely on manual tuning or controller randomization, which can be labor-intensive, task-specific, and introduce significant training difficulty. In this work, we propose a framework that jointly learns actions and controller parameters based on the historical information of both trajectory and controller. This adaptive controller adjustment mechanism allows the policy to automatically tune control parameters during execution, thereby mitigating the sim-to-real gap without extensive manual tuning or excessive randomization. Moreover, by explicitly providing controller parameters as part of the observation, our approach facilitates better reasoning over force interactions and improves robustness in real-world scenarios. Experimental results demonstrate that our method achieves improved transfer performance across a variety of dexterous tasks involving variable force conditions.

==> Tables/flipping_table.tex <==
\begin{table}[t]
% \vspace{6pt}
\begin{minipage}{0.48\textwidth}
\caption{Quantitative results of oracle policy for rotation in the simulation.
}
\vspace{6pt}
\centering
% \small
\footnotesize 
\setlength{\tabcolsep}{12pt}
% \renewcommand{\arraystretch}{1.0}
\begin{threeparttable}
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|c|c|c|c}
\toprule
% \multirow{2}{*}{ Method }   & \multicolumn{2}{c}{ General Set } & \multicolumn{2}{c}{ Hard Set } \\ 
 & Method & RotR $\uparrow$ & TTF $\uparrow$ & ObjVel $\downarrow$\\
\midrule
% Method & Metrics & Light(44g)  & Medium(94g) & Heavy(160g) & Small & Medium & Large \\ 
\multirow{3}{*}{\makecell{With\\Disturbance}} 
& Manual Tuning & 21.02 & 0.285 & 134.6 \\
& Ours w/o PD & 22.77 & 0.287 & 136.0 \\
& Ours & 23.34 & 0.237 & 174.5 \\
   % & Top1 & Top5 & Top1 & Top5  \\  
% \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-6}
\midrule
% \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5}

\multirow{3}{*}{\makecell{Without\\Disturbance}} 
& Manual Tuning & 40.09 & 0.162 & 204.6 \\
& Ours w/o PD & 46.15 & 0.156 & 221.1 \\
& Ours & 48.04 & 0.140 & 274.3 \\

\bottomrule
\end{tabular}
}
\end{threeparttable}
\label{table:sim}
% \vspace{-20pt}
\end{minipage}
\end{table}
